Heuristic-based Inter-training to Improve Few-shot Multi-perspective Dialog Summarization

Many organizations require their customer-care agents to manually summarize their conversations with customers. These summaries are vital for decision making purposes of the organizations. The perspective of the summary that is required to be created depends on the application of the summaries. With this work, we study the multi-perspective summarization of customer-care conversations between support agents and customers. We observe that there are different heuristics that are associated with summaries of different perspectives, and explore these heuristics to create weak-labeled data for intermediate training of the models before fine-tuning with scarce human annotated summaries. Most importantly, we show that our approach supports models to generate multi-perspective summaries with a very small amount of annotated data. For example, our approach achieves 94\% of the performance (Rouge-2) of a model trained with the original data, by training only with 7\% of the original data.

==> sections/2_related_work.tex <==
\section{Related Work}

Some previous work have attempted to address the few shot learning problem in abstractive summarization. \citet{bravzinskas2020few} exploited summary related properties
in unannotated reviews that can be conditioned on during the training of the summary generator. \citet{magooda2021exploring} show that in low resource scenarios, a model trained in a multitask setting outperforms a model trained only for abstractive summarization, with no additional summarization
data introduced. In \citet{parida2019abstract, gunasekara-etal-2021-summary} generating synthetic data is used to improve summarization accuracy in low resource scenarios, where to generate synthetic data, they train a system in the reverse direction (i.e. source as summary and target as text). \citet{magooda2020abstractive} use a method which first extract templates from provided summaries and  then inject keywords into a template and perform rewriting into a coherent summary to improve performance in low resource scenarios. 
\citet{goyal2021hydrasum} focuses on creating different versions of a summary using multiple decoders. However this is different from the multi-perspective summaries that we study. 

